DiGamma: Domain-aware Genetic Algorithm for HW-Mapping Co-optimization for DNN Accelerators

The design of DNN accelerators includes two key parts: HW resource configuration and mapping strategy. Intensive research has been conducted to optimize each of them independently. Unfortunately, optimizing for both together is extremely challenging due to the extremely large cross-coupled search space. To address this, in this paper, we propose a HW-Mapping co-optimization framework, an efficient encoding of the immense design space constructed by HW and Mapping, and a domain-aware genetic algorithm, named DiGamma, with specialized operators for improving search efficiency. We evaluate DiGamma with seven popular DNNs models with different properties. Our evaluations show DiGamma can achieve (geomean) 3.0x and 10.0x speedup, comparing to the best-performing baseline optimization algorithms, in edge and cloud settings.

==> figure/design_space.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth]{Figures/design_space.pdf}
\end{center}
\vspace{-0.3cm}
\caption{An illustrative example of the potential performance difference of the found solutions by different accelerator design schemes. Fixed HW/Mapping: A manual-designed fixed HW and mapping. HW-opt: A manual-tuned fixed mapping with HW search. Mapping-opt: A manual-tuned fixed HW configuration with mapping search. HW/Map-co-opt: A framework searching for both HW and mapping simultaneously.}

\label{fig:design_space}
\end{figure}




==> figure/exp.tex <==
\begin{figure*}[t]
\begin{center}

\includegraphics[width=1\linewidth]{Figures/exp_short.pdf}
\end{center}
\vspace{-0.3cm}
\caption{The performance comparisons of \system (\digamma) and a hand-optimized baseline DLA-like accelerator (dla) across different DNNs over edge and cloud settings. Area evaluated under process point 14nm. }
\vspace{-0.7cm}
\label{fig:exp}
\end{figure*}




==> figure/exp_cloud.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=1\linewidth]{Figures/exp_cloud.pdf}
\end{center}
\vspace{-0.3cm}
\caption{The found solutions on cloud accelerator resources.}

\label{fig:exp_cloud}
\end{figure*}




==> figure/exp_edge.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=1\linewidth]{Figures/exp_edge.pdf}
\end{center}
\vspace{-0.3cm}
\caption{The found solutions on edge accelerator resources.}

\label{fig:exp_edge}
\end{figure*}




==> figure/exp_others_latency.tex <==
\begin{figure}[t]
\begin{center}

\includegraphics[width=1\linewidth]{Figures/exp_others_latency.pdf}
\end{center}
\vspace{-0.3cm}
\caption{}
\vspace{-0.7cm}
\label{fig:exp_others_latency}
\end{figure}




==> sections/03-Approach-old.tex <==
\input{figure/toolflow}
\input{figure/system}

\section{Technical Approach}
\label{sec:methodology}
%We propose a mapping-HW co-optimization method called \system, standing for the the next generation of the open-source tool GAMMA. \system provides a sample-efficient solution for mapping-HW co-optimization for DNN accelerator design.

\textbf{Problem Formulation.}  \emph{Under a chip area budget and given a DNN model, we aim to design an accelerator with optimized HW resource allocation for PEs, local buffer (L1), and global buffer (L2), and an optimized mapping strategy.}
\vspace{-1mm}
\subsection{Genetic Algorithm}

\textbf{Baseline Genetic Algorithm.}
A baseline Genetic Algorithm (GA) consist of two phases: evaluation (evaluate the performance/ fitness of a bag of candidate solutions) and evolution (select the good candidates and reproduce the next bag of candidate with genetic operators). In GA, we often call a parameter of a candidate: a \text{gene}, each candidate: an \textit{individual}, a bag of candidates: a \text{population}, and one iteration of running the two phases (evaluation and evolution): a \textit{generation}. In evolution phase, baseline GA has two standard genetic operators: crossover (blend the genes of individuals and reproduce populations for next generation) and mutation (perturb the genes of each individual).

%\textbf{Why GA?}
\textbf{GAMMA.}
Research shows GA reaches competitive performance with deep reinforcement learning \cite{uberGA,openai_es}, and hyper-parameter optimization problem.  STOKE \cite{schkufza2013stochastic} and Tensor Comprehensions \cite{vasilache2018tensor} use GA to optimize DNN compute flow. Comparing to many optimizations methods, GA is light, fast, and highly parallelizable ~\cite{uberGA, openai_es}. However, the key challenge is it's sample efficiency.
%
%\textbf{GAMMA.}
GAMMA~\cite{gamma} is an open-source mapping search tool~\cite{gamma_web} using several specialized genetic operators to specifically explore different knobs of mapping (tiling, order, parallelism) and shows high sample efficiency. The inputs of GAMMA includes: a target DNN model, an objective (e.g., minimum latency),  and a HW resources configuration. This tool is useful for mapping exploration at compile-time when the the underlying accelerators are fixed, however, challenging at design-time when designing a new DNN accelerator, where the HW resources are not fixed and are part of the tuning parameters.
% This long search time problem is also a well-known challenge in NAS related research~\cite{nas}. 

\subsection{\system High-level Overview}
We integrate the two searching loops (\autoref{sec:challenge}), HW and mapping, into one unified optimization process. The input and output of the \system are shown in \autoref{fig:toolflow}. When \system starts, it executes the algorithm flow in \autoref{fig:system}(a).
%\system includes evolution and evaluation part.
At the start, it randomly initializes a population of individuals.
Each individual \textit{encodes} a design-point 
and comprises of genes to represent both HW resources and mapping (\autoref{sec:components}).
All individuals go through genetic operators housed in the evolution part, where the genes get perturbed. Then the evaluation starts. The genes of each individual are \textit{decoded} into an accelerator design point.
%as shown in \autoref{fig:system}(b)(d).
\system inputs each design point into the HW performance evaluator to collect its HW performance (e.g., latency, power), assigns it a fitness value, select the individuals with good fitness values and not violating constraint to enter next generation, and the whole iteration starts again. The algorithm stops when it reaches the sampling budgets (number of data points allowed to be sampled in the optimization process). 






% The fitness value is decided by the considered objective. For example minimum latency as the objective, the fitness value will be the latency value of the evaluating accelerator configuration. 


\subsection{\system Components}
\label{sec:components}
We discuss the major components of \system as follows.



\subsubsection{\textbf{Genetic Encoding: Design Space Description}}
We develop a customized encoding as shown in \autoref{fig:system}(b-c) (notation shown in \autoref{fig:system}(g)) to describe an accelerator design-point. 
%design space description with a series of encoding values, termed genetic encoding in our GA-based algorithm, as shown in \autoref{fig:system}(b-c) (notation definition is shown in \autoref{fig:system}(g)).
Our encoding also captures the memory hierarchy. %Different level of configurations show the HW and mapping of different hierarchy levels in the accelerator.
We show a 2-hierarchy level accelerator in \autoref{fig:system}(b-c) as an example. Each key-value pair represents a gene. L1-config (yellow) shows the accelerator configuration (HW and mapping) of a 1-D PE array. $\pi_{L1}$, a HW parameter, shows the length of the 1-D PE array. The rest of the genes ($P$,$C$,$K$,$Y$,$X$,$R$ and $S$) describe the mapping parameters for the 1-D PE array, including tiling, order, and parallelism. 
The value genes describe the tile sizes of the corresponding key dimension.
Order of key genes describes the compute order. $P$ gene tells the dimension to parallelize the compute across 1-D PE array. L2-config shows the HW and mapping across several 1-D PEs arrays, effectively describing a  2-D PE arrays. $\pi_{L2}$, a HW parameter, shows the number of instantiated 1-D PE array, while the rest mapping genes decide the mapping parameters across 1-D PE arrays. Similarly, a 3-level hierarchy (i.e., several 2D arrays) can also be described.
%\footnote{Note that if we have deeper hierarchy of config, e.g., 3-level config, the L3-config will dictate the HW and mapping across 2-D PEs arrays, which could be multiple parallel 2-D PEs arrays or an actual stacked 3-D PEs arrays, depending on the implementation.}.

\subsubsection{\textbf{Genetic Decoding: Design Point Derivation}}
When evaluating the fitness/performance of each individual's genes, we decode them back to an exact accelerator design point. \autoref{fig:system}(d) shows the decoded accelerator design point for genes in \autoref{fig:system}(b). The $\pi_{L2}$ and $\pi_{L1}$ decide the PE array sizes and aspect ratio, as shown in \autoref{fig:system}(f). The $P$ values of L2 and L1 implies a K-C parallelism strategy (similar to NVDLA~\cite{nvdla}) across the PE array. PE array sizes and tiling sizes together decide the sizes of weight, input, and output tiles, which decides the \textit{minimum buffer requirement} for weight, input, and output buffer at both L2 and L1, and becomes the the most optimized buffer allocations that \system allocates to the design point.

% \subsubsection{\textbf{Minimum Buffer Requirement as Buffer Allocation}}\FK{Move into decoding part.}
% The formula in \autoref{fig:system}(f) shows the calculation of minimum buffer requirement, defined as follows: \emph{the minimum on-chip buffer size to hold the data to serve the current accelerator configurations without going to off-chip memory while executing the computation.} As a mapping-HW co-search process, \system always instantiates/ allocates the minimum possible buffer sizes, decided by formula in \autoref{fig:system}(f), to maximize the buffer resource efficiency. 

\subsubsection{\textbf{Fitness Evaluation}}

\textbf{(a) HW Performance Evaluator.}
We evaluate the design points by an open-source HW performance evaluator, MAESTRO~\cite{maestro_web}, which has detailed micro-architectural HW models validated against chip prototypes~\cite{maestro}.  MAESTRO takes in the accelerator design (HW and mapping) and outputs a detailed HW performance report including latency, area, power, energy, and so on.
%We extract the related performance (latency, HW resources area (area)).
We use HW resource area as constraint which includes PEs, L1 and L2 buffers area\footnote{\label{sec:area_footnote}A complete chip area will also includes NoCs, logics, routing, clock trees, pin placement, and others, which need other physical layout considerations and are not considered in MAESTRO and this paper.}. In this work, we use latency as fitness and area as constraint.

\textbf{(b) Constraint Check.}
In constraint checker, if the reported area of the current design point is larger than the area constraint budget, we invalidate the design point by re-assigning it a negative fitness value, so that it won't be selected as one of the candidates to enter the next generation, as shown in ~\autoref{fig:system}(a).



\subsubsection{\textbf{Genetic Operators}}
%Genetic operators includes crossover, mutations and others.
Rather than using conventional genetic operators (crossover, mutations) to perturb the genes arbitrarily, we develop specialized genetic operators for individual HW and mapping genes to capture the structure of the design space.
%We specifically design domain-aware genetic operators for different HW and mapping parameters,
The genetic operators, responsible for mapping, are modified from GAMMA~\cite{gamma}. We add a \textit{HW} genetic operator --- a PE mutation operator. The PE mutation operator will perturb the values of $\pi_{L2}$ and $\pi_{L1}$, which change the total number of PEs and the aspect ratio of PE array. 
Thus each gene 
%have the notion of the structure of the design space for the give and know how to 
can step through and explore the design-space efficiently. \footnote{The hyper-parameters of \system, (mutation rate, crossover rate, elite ratio, population size to number of generations ratio, and so on), are decided by a Bayesian optimization-based %hyper-parameter 
search process~\cite{bayes_python}.}

\begin{comment}
There are six steps enabling the extension of a mapping optimizer to a mapping-HW co-optimizer, described as follows.

\subsubsection{\textbf{Relieving underlying HW Assumption}}
The configuration of HW resources is an input of a mapping optimizer, which defines the available HW resources of the underlying HW accelerator and constrains the search space of the mapper. To enable the exploration of HW resource together, we remove this HW resource constraints. To be more specific, we disable the input argument of HW resources configurations of a mapper and allow the algorithm to explore any sizes of HW resources.

\subsubsection{\textbf{Genetic Encoding for PE}}
We inherent the genetic encoding inside GAMMA for the inner-loop (mapping) part and extend it with the genetic encoding of outer-loop (HW) part. Specially, we add a PE gene, which describe the number of PEs to run the current mapping (inner-loop).

\subsubsection{\textbf{Genetic Operator for PE}}
We add a PE mutation operator, which mutate the number of PEs of an individual. To explore PE configuration with efficiency, we did not use random sampling for exploring the PEs. Instead, we apply a mapping-aware PE configuration sampling. Note that the underlying assumption for the PEs array is that it is a 2D PEs array, which can explore two-level of parallelism (across height and width of the array). The L2-mapper in \autoref{fig:system} describes the mapping across width and the L1-mapper describes the mapping across height. Hence, the number of parallelism of L1-mapper, the first gene value of L1-mapper, will determine the height of the PEs array, while the width of the PEs array is implicitly determine by the total number of PEs. Therefore, in our case, when we explore the number of PEs by the PE mutation operator, we specifically choose to explore the width of the PE array while the height is fixed by the mapping, i.e., we only allow the mutation operator to explore the values that are the multiply of the height. The reason is that all the intermediate values for the PE configuration will only introduce redundant PEs, which wastes the HW resources and could not improve the latency performance. This mapping-aware PE mutation could largely reduce the redundant search space.


\subsubsection{\textbf{Backward-compatibility of Other Mapping Operators}}
Likewise, for other genetic operators for mapping exploration, we also need to enable HW-aware mapping mutation. Whenever the mapping mutation operator choose to mutate the parallelism size of L1-mapper, it will reference the current number of PEs and restrict the search space of parallelism size to the factor of the number of PEs. The non-factor values will cause waste of PEs and reduce the latency performance. 


\subsubsection{\textbf{Memory Footprint as Buffer Assignment}}
\label{sec:buffer_explain}
As mentioned previously, we eliminate the HW resource constraint From the perspective of buffer, we allow the algorithm to explore any sizes of SL and SG. Instead, we track the live memory footprint \footnote{The minimum buffer requirement to hold the data to avoid going to off-chip memory when executing the current mapping with current PEs} of both SL and SG and output them as the buffer requirements. 

\subsubsection{\textbf{Area as a Constraint}}
The chip area for the corresponding PE and buffer resources becomes the constraint. \system takes the chip area size constraint as input. \system tracks the area sizes of each individual and invalidate the individual exceeding the area constraint by assigning it a negative infinite fitness value at the evaluation phase. Note that in this work, we study the chip area usage of the major HW components of DNN accelerators ( PEs, SL, and SG), while the actual packaged chip area will also includes NoCs, logics, routing, clock trees, pin placement, and others, which need other physical layout considerations and are not the focus of this paper. 

\subsection{Walk-through Example}
The input and output of the \system are shown in \autoref{fig:toolflow}. \system takes in a targeting DNN model, optimizing objective (e.g., minimum latency), and the chip area budget. \system outputs an accelerator configuration including the allocated HW resources and its optimized mapping. \system also outputs a report of the performance of the found accelerator such as latency, area, power, and energy. An example solution of accelerator configuration is shown in \autoref{fig:system}(a), which is also a NVDLA-like~\cite{nvdla} accelerator description. The key represent dimensions, and values represent sizes of tiling, number of parallelism, or number of PEs. The first gene value of L2-mapper shows that the total number of PEs are 1,024. The first gene value of L1-mapper shows that the height of PE array is 64, implying the shape of PEs array 64x16. The first gene key of L2 and L1 mapper show that this is a K-C parallelism mapping (NVDLA-like), whose HW implication is shown in \autoref{fig:system}(b) and notation deneition is shown in \autoref{fig:system}(c). For the 2nd to 7th genes of both mapper shows the compute order and the tile sizes of different dimensions. 
\end{comment}

==> sections/05-RelatedWork.tex <==
\section{Related Work}

\textbf{HW Resources Allocations Optimizations.}
The HW resource allocation problem has been widely-studied in the FPGA community~\cite{hao2019fpga,zhong2017design,motamedi2016design,shen2017maximizing,zhang2016energy,zhang2018dnnbuilder,chen2019cloud,jiang2018heterogeneous,li2016high,jiang2019xfer, wei2018tgpa,jiang2019achieving}. With the fast-growing of DNN/ML researches, the DNN ASIC accelerator design starts to find the need of autonomous optimization methods to assisted the accelerator design for speeding-up chip design time~\cite{santoro2018energy, minerva, aladdin,cong2018polysa, wei2017automated}. Recently, more and more ML techniques are integrated in the chip design process, such as reinforcement learning (RL) ~\cite{confx,mirhoseini2020chip} and GNN~\cite{wang2020gcn}.



\textbf{Mapping Optimizations.}
Many mapping optimization methods have been proposed. Techniques includes: formulating a more comprehensive design space for better capturing the accelerator behavior~\cite{gamma, timeloop, simba}, improving the design space description for search efficiency~\cite{yang2020interstellar, dmazerunner,deeptools}, and incorporating different ML techniques in the optimization process~\cite{ahn2019reinforcement, reagen2017case,chen2018tvm,autotvm,suda2016throughput,vasilache2018tensor}. 

These prior efforts focus on the optimization of either HW or mapping independently. In this work, we co-optimize the mapping and HW together.




==> table/cloud_table.tex <==


\begin{table}[h]

\centering
\caption{The experiment results on cloud platform on Heteto (S4) and Hetero BigLittle (S5) setting. }

\includegraphics[width=1\linewidth]{Figures/cloud_graph.pdf}
% Figures/cloud_table.pdf
\vspace{-0.5cm}
\label{table:cloud_table}
\end{table}


==> table/edge_bw_effect.tex <==


\begin{table}[h]

\centering
\caption{The latency decrease with the increase of BW budget on (a) S1 and (b) S2.}

\includegraphics[width=1\linewidth]{Figures/edge_bw_effect.pdf}
\vspace{-0.2cm}
\label{table:edge_bw_effect}
\end{table}


==> table/edge_table.tex <==


\begin{table*}[h]

\centering
\caption{The experiment results on fog node with (a) S1 and (b) S2 setting, and on cloud node on (c) S4 and (d) S5 setting. }

\includegraphics[width=1\linewidth]{Figures/edge_graph.pdf}
% Figures/edge_table.pdf
\vspace{-0.2cm}
\label{table:edge_table}
\end{table*}


==> table/ga_table.tex <==


\begin{table}[t]

\centering
\caption{Terminology in \system Genetic Algorithm (GA).}
%\TK{It would be great if in this table, Gene can be defined for what it means in G-SHARP. Similarly, genome uses the word feature which is not defined.}\FK{Fixed.}}

\includegraphics[width=1\linewidth]{Figures/ga_table.pdf}
\vspace{-0.5cm}
\label{table:ga_terminology}
\end{table}


==> table/highlevel_comparison.tex <==

\begin{table}[t]

\centering
\caption{ The comparisons of related works on multi-tenancy and multi-sub-accelerators. }

\includegraphics[width=1\linewidth]{Figures/highlevel_comparison.pdf}
% Figures/cloud_table.pdf
\vspace{-0.5cm}
\label{table:highlevel_comparison}
\end{table}


==> table/model_table.tex <==


\begin{table}[h]

\centering
\caption{Models of different applications included in the experiments. }

\includegraphics[width=1\linewidth]{Figures/model_table.pdf}
% Figures/cloud_table.pdf
\vspace{-0.5cm}
\label{table:model_table}
\end{table}


==> table/model_table_latex.tex <==

\begin{table}[]
\caption{\it Evaluated DNNs in different applications.}
\scriptsize
% \begin{tabular}{|
% >{\columncolor[HTML]{EFEFEF}}c |l|}
\begin{tabular}{|>{\columncolor[HTML]{C0C0C0}}p{2.0em}|p{31em}|}
\hline
App Type & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}DNN Models}                                                                                                                                   \\ \hline
Vision   & \makecell[l]{AlexNet~\cite{Alexnet}, DenseNet~\cite{densenet}, GoogleNet~\cite{Googlenet}, MnasNet~\cite{mnasnet}, \\ MobileNet-V2~\cite{sandler2018mobilenetv2},  ResNet50~\cite{Resnet}, ResNext50~\cite{resnext},  ResNet18~\cite{Resnet},\\  WideResNet50~\cite{Resnet}, SuffleNet-V2~\cite{zhang2018shufflenet},  SqueezeNet~\cite{squeezenet}, VGG16~\cite{vgg}  }                                                 \\ \hline
Lang & \makecell[l]{ALBERT~\cite{albert}, Bart~\cite{bart}, BERT~\cite{bert}, CamemBERT~\cite{camembert}, CTRL~\cite{ctrl_lang},\\ DistilBERT~\cite{sanh2019distilbert}, ELECTRA~\cite{electra}, FlauBERT~\cite{flaubert}, GPT2~\cite{gpt2}, GPT~\cite{gpt},\\ LongFormer~\cite{longformer}, MarianNMT~\cite{mariannmt}, MobileBERT~\cite{sun2020mobilebert}, Reformer~\cite{reformer}, \\ RetriBERT~\cite{retribert}, RoBERTa~\cite{roberta}, T5~\cite{t5}, TransformerXL~\cite{transformerxl}, XLM~\cite{xlm}, \\ XLM-RoBERTa~\cite{xlmroberta}, XLNet~\cite{xlnet}} \\ \hline
Recom    & \makecell[l]{DIN~\cite{din}, DIEN~\cite{dien},  DLRM-MLPerf~\cite{mlperf}, DLRM-large~\cite{dlrm_intel}, \\DLRM-small~\cite{dlrm}, WideDeep~\cite{widedeep}, DLRM-RMC1~\cite{deeprecsys}, DLRM-RMC2~\cite{deeprecsys} }                                                                                                         \\ \hline
\end{tabular}
\label{table:model_table}
\end{table}

==> table/opt_table.tex <==

\begin{table}[t]

\centering
\caption{Baseline heuristics and optimization methods. Green rows represent heuristics for job prioritizing or accel selection. A complete schedule algorithm is the combination of two. e.g., FCFS-OLB. HEFT is a state-of-the-art   joint method. Blue rows represent a list of baseline optimization methods, which jointly optimize both aspects.}

\includegraphics[width=1\linewidth]{Figures/opt_table_with_parameter.pdf}
\vspace{-0.4cm}
\label{table:opt_table}
\end{table}



==> table/programmable_table.tex <==


\begin{table}[t]

\centering
\caption{The traffic analysis of different level of flexibility and their latency performance. }

\includegraphics[width=1\linewidth]{Figures/programmable_table_graph.pdf}
% Figures/programmable_table.pdf
\vspace{-0.2cm}
\label{table:programmable_table}
\end{table}


==> table/s3_s4_s5.tex <==
\begin{table*}[h]

\centering
\caption{(a) The averaged non-stall latency and the required BW of S3 (BigHomo), S4 (BigHetero), and S5 (BigLittleHetero) in different traffics. (b) The latency performance for S3, S4, and S5 in different traffics and BW. }

\includegraphics[width=1\linewidth]{Figures/s3_s4_s5_graph.pdf}
% Figures/s3_s4_s5.pdf
\vspace{-1cm}
\label{table:s3_s4_s5}
\end{table*}


==> table/s6.tex <==


\begin{table*}[h]

\centering
\caption{The experiment results on cloud platform on Scale-up (S6), BW=1. }

\includegraphics[width=1\linewidth]{Figures/s6.pdf}
\vspace{-0.2cm}
\label{table:s6_table}
\end{table*}


==> table/setting.tex <==

\begin{table}[t]
\vspace{-0.2cm}
\centering
\caption{Platform setting of the experiments.}

\includegraphics[width=1\linewidth]{Figures/setting.pdf}
\vspace{-0.6cm}
\label{table:setting}
\end{table}



==> table/traffic_analysis.tex <==


\begin{table*}[h]

\centering
\caption{Traffic analysis of different applications. }

\includegraphics[width=1\linewidth]{Figures/traffic_analysis.pdf}
\vspace{-0.2cm}
\label{table:traffic_analysis}
\end{table*}


==> table/trf.tex <==


\begin{table}[t]

\centering
\caption{The performance of knowledge transferring on (a) Mix, setting S4, BW=1, and (b) the averaged performance across different applications and different settings under BW=1. All the values are normalized by the values of Trf-100-ep of each columns. Raw (highlighted in orange) is the latency without learning or transferred. Trf-0-ep (highlighted in green) is a direct transfer. Trf-1-ep is a transfer with one epoch of re-training, and likewise for Trf-30-ep. Trf-100-ep (highlighted in blue) is a full training.}

\includegraphics[width=1\linewidth]{Figures/trf.pdf}
\vspace{-0.5cm}
% \RaggedRight
% \begin{justify}
% \footnotesize \dag All the values are normalized by the values of Trf-100-ep of each columns. Raw is the latency without learning or transferred. Trf-0-ep is a direct transfer without retraining. Trf-1-ep is a transfer with one epoch of re-training, and likewise for Trf-30-ep and Trf-100-ep. Since we run all the optimization for 100 epochs, Trf-100-ep is similar to training from scratch.
% \end{justify}
\label{table:trf}
\end{table}



==> table/trf_1.tex <==


\begin{table}[t]

\centering
\caption{The knowledge transferring on Vision, S4 setting. All the values are noramalized by the values of Trf-100-ep of each columns. Raw is the latency without learning or transferred. Trf-0-ep is a direct transfer without retraining. Trf-1-ep is a transfer with one epoch of re-training, and likewise for Trf-30-ep and Trf-100-ep.Since we run all the optimization for 100 epochs, Trf-100-ep is similar to training from scratch. }

\includegraphics[width=0.7\linewidth]{Figures/trf_1.pdf}

\label{table:trf_1}
\end{table}


==> table/trf_2.tex <==


\begin{table}[h]

\centering
\caption{The knowledge transferring on (left) different setting of Mix traffics and (right) different traffic types. All the values are noramalized by the values of Trf-100-ep of each columns.}

\includegraphics[width=1\linewidth]{Figures/trf_2.pdf}

\label{table:trf_2}
\end{table}

